Nominal Equational Rewriting and Narrowing

Narrowing is a well-known technique that adds to term rewriting mechanisms the required power to search for solutions to equational problems. Rewriting and narrowing are well-studied in first-order term languages, but several problems remain to be investigated when dealing with languages with binders using nominal techniques. Applications in programming languages and theorem proving require reasoning modulo alpha-equivalence considering structural congruences generated by equational axioms, such as commutativity. This paper presents the first definitions of nominal rewriting and narrowing modulo an equational theory. We establish a property called nominal E-coherence and demonstrate its role in identifying normal forms of nominal terms. Additionally, we prove the nominal E-Lifting theorem, which ensures the correspondence between sequences of nominal equational rewriting steps and narrowing, crucial for developing a correct algorithm for nominal equational unification via nominal equational narrowing. We illustrate our results using the equational theory for commutativity.

==> eptcsdata.tex <==
\providecommand{\firstpage}{80}
\providecommand{\publicationstatus}{Cynthia Kop and Helida Salles Santos (Eds); 19th Workshop on\\ Logical and Semantic Frameworks with Applications (LSFA'24)\\
EPTCS 421, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.421.5}{10.4204/EPTCS.421.5}}
\pdfoutput=1

